A Framework for Exploring the Consequences of AI-Mediated Enterprise Knowledge Access and Identifying Risks to Workers

Organisations generate vast amounts of information, which has resulted in a long-term research effort into knowledge access systems for enterprise settings. Recent developments in artificial intelligence, in relation to large language models, are poised to have significant impact on knowledge access. This has the potential to shape the workplace and knowledge in new and unanticipated ways. Many risks can arise from the deployment of these types of AI systems, due to interactions between the technical system and organisational power dynamics. This paper presents the Consequence-Mechanism-Risk framework to identify risks to workers from AI-mediated enterprise knowledge access systems. We have drawn on wide-ranging literature detailing risks to workers, and categorised risks as being to worker value, power, and wellbeing. The contribution of our framework is to additionally consider (i) the consequences of these systems that are of moral import: commodification, appropriation, concentration of power, and marginalisation, and (ii) the mechanisms, which represent how these consequences may take effect in the system. The mechanisms are a means of contextualising risk within specific system processes, which is critical for mitigation. This framework is aimed at helping practitioners involved in the design and deployment of AI-mediated knowledge access systems to consider the risks introduced to workers, identify the precise system mechanisms that introduce those risks and begin to approach mitigation. Future work could apply this framework to other technological systems to promote the protection of workers and other groups.

==> harm_mechanisms_table.tex <==
\begin{table}[]
\caption{Overview of the consequences and the related system mechanisms that introduce risk to workers from AI-mediated EKA.}
\label{table-harm mechanisms}
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Consequence}        & \textbf{Mechanism}                                                                 & \textbf{Description}                                                                                                                                                                                                                                                                                                                                             & \textbf{Specific Example}                                                                                                                                                                                                                                                                          \\ \hline
\textbf{Commodification} & \begin{tabular}[c]{@{}l@{}}Disturbed \\ Relationality\end{tabular}                  & \begin{tabular}[c]{@{}l@{}}The acts of removing know-\\ ledge artifacts out of the \\ relational context in which \\ they exist or are produced, \\ including who produced \\ them, the social and proce-\\ dural context in which they\\ are produced, and the context \\ of other knowledge artifacts \\ in which they exist or were \\ produced.\end{tabular} & \begin{tabular}[c]{@{}l@{}} A system may not maintain \\ the provenance of informa- \\ tion, such as author, if it is an \\ LLM that is trained directly\\  on enterprise data and inter- \\ acted with directly.\end{tabular}                                                                                                                                                                              \\ \cline{2-4} 
\textbf{}                & \begin{tabular}[c]{@{}l@{}}Changing \\ Value\end{tabular}                           & \begin{tabular}[c]{@{}l@{}}The acts that lead to \\ systemic departure in \\ valuation of knowledge \\ artifacts compared to their \\ existing and historical \\ valuation.\end{tabular}                                                                                                                                                                       & \begin{tabular}[c]{@{}l@{}}A system may value types of\\ knowledge that are qualitative \\ e.g. if a worker is skilled at \\ debugging, this type of \\knowledge will not be captured \\ as it is hard to infer from \\written documents.\end{tabular}                                                                                                                                         \\ \cline{2-4} 
\textbf{}                & \begin{tabular}[c]{@{}l@{}}Shifting Focus \\ from Praxis \\ to Proxies\end{tabular} & \begin{tabular}[c]{@{}l@{}}The acts of creating an \\ environment where \\ workers are encouraged \\ to focus more on optim-\\ izing towards (often top-\\ down) pre-stated quantitative \\ measures of   outcomes \\ (proxies) over (ideally \\ bottom-up) reflection and \\ action directed at the \\ outcome to be transformed.\end{tabular}                  & \begin{tabular}[c]{@{}l@{}} A system may use number of \\ contributions on a subject as a  \\ proxy metric for expertise. This  \\ could incentivise workers to  \\ write documentation for the   \\ system as opposed to practising  \\ their expertise. \end{tabular}                                                                                                                                                                 \\ \cline{2-4} 
\textbf{}                & \begin{tabular}[c]{@{}l@{}}Commensuration \\ and \\ Standardisation \end{tabular}                                                         & \begin{tabular}[c]{@{}l@{}}The acts of transforming \\ different qualities into \\ a common metric and enforcing \\ conformity over things that \\  are not strictly similar.\end{tabular}                                                                                                                                                                                                                                                 & \begin{tabular}[c]{@{}l@{}}A system may adopt a \\ standard schema to represent all\\ entities of a specific type, dis-\\ regarding the knowledge about\\ individual entities that can’t fit \\ into the schema.\end{tabular} \\ \cline{2-4} 
% \textbf{}                & Standardisation                                                                     & \begin{tabular}[c]{@{}l@{}}The acts of enforcing \\ conformity over things \\ that are not strictly \\ similar.\end{tabular}                                                                                                                                                                                                                                     & \begin{tabular}[c]{@{}l@{}}A knowledge base may adopt a \\ standard schema to represent all\\ entities of a specific type, dis-\\ regarding the knowledge about\\ individual entities that can’t fit \\ into the schema.\end{tabular}                                                              \\ \cline{2-4} 
\textbf{}                & Homogenisation                                                                      & \begin{tabular}[c]{@{}l@{}}The process of making \\ things uniform or \\ similar.\end{tabular}                                                                                                                                                                                                                                                                   & \begin{tabular}[c]{@{}l@{}}If   workers are incentivized to \\ make their content more easily \\ extractable by an automated \\ system that may lead to homo-\\ genization of their authoring  \\ style   towards what the machine \\ can best extract from.\end{tabular}                           \\ \hline
\textbf{Appropriation}   & \begin{tabular}[c]{@{}l@{}}  Knowledge \\ Extractivism \end{tabular}                   & \begin{tabular}[c]{@{}l@{}}The process of \\ extracting knowledge \\ and co-opting it as the \\ system's own.\end{tabular}                                                                                                                                                                                                                                       & \begin{tabular}[c]{@{}l@{}}A system  may surface a summ-\\ ary of a document without \\ recognition of the original auth- \\ or, obscuring their labour.\end{tabular}                                                                                                                           \\ \hline
\end{tabular}
\end{table}


\begin{table}[]
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Dimension of Risk}                                                           & \textbf{Mechanism}                                                                                  & \textbf{Description}                                                                                                                                                                                                                                                                                                           & \textbf{Specific Example}                                                                                                                                                                                                                                                                                                                      \\ \hline
\textbf{Appropriation}                                                      & \begin{tabular}[c]{@{}l@{}}Capture of \\ Information\end{tabular}                                    & \begin{tabular}[c]{@{}l@{}}The acts of establishing \\ exclusive control over \\ certain knowledge \\ artifacts.\end{tabular}                                                                                                                                                                                                  & \begin{tabular}[c]{@{}l@{}}A system may recognize \\ relationships between different \\ topics based on patterns of \\ how users interact with them, \\ rather than based on what is \\ documented in the content.\end{tabular}                                                                                                               \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Concentration \\ of Power\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Reduced space \\ for Negotiation\end{tabular}                             & \begin{tabular}[c]{@{}l@{}}Reduced space for neg-\\ otiation refers to the acts \\ that shrink the set of \\ decisions that workers \\ can meaningfully contri-\\ bute to or contest.\end{tabular}                                                                                                                             & \begin{tabular}[c]{@{}l@{}}In the problem of expert identi-\\ fication, a system may \\ replace social  processes with \\ alternative computational appr-\\ oaches that take away any say \\ the workers previously had in \\ this context and limited \\ contestation.\end{tabular}                                                      \\ \cline{2-4} 
\textbf{}                                                                   & \begin{tabular}[c]{@{}l@{}}Worker \\ Dispossession\end{tabular}                                      & \begin{tabular}[c]{@{}l@{}}Worker dispossession \\ refers to the acts of \\ depriving workers of \\ their job opportunities, \\ skills, and expertise \\ status.\end{tabular}                                                                                                                                                  & \begin{tabular}[c]{@{}l@{}}A system may change a deve- \\ loper's role to spend more time \\ developing content for the KB  \\ instead of writing code, as the   \\ system is better at recognising \\ documents than python scripts.\end{tabular}                                                                                         \\ \cline{2-4} 
\textbf{}                                                                   & System Opacity                                                                                        & \begin{tabular}[c]{@{}l@{}}System opacity refers \\ to the acts of intentional \\ and unintentional obfu-\\ scation of how systems \\ work under the hood. \end{tabular} & \begin{tabular}[c]{@{}l@{}}Workers do not know what \\information about them a \\system collects and what may \\be inferred from it. \end{tabular}                                                                                                                                                                             \\ \hline
\textbf{Marginalization}                                                    & \begin{tabular}[c]{@{}l@{}}Systemic \\ Reproduction \end{tabular} & \begin{tabular}[c]{@{}l@{}}The acts that lead to marg-\\ inalization of the same \\ groups who have been \\ historically discriminated \\ against and marginalized\\  by society (or the \\ organization).\end{tabular}                                                                                                        & \begin{tabular}[c]{@{}l@{}}A system may reproduce hist-\\ orical marginalization by race \\ if it fails to adequately handle \\ linguistic differences between \\ groups because it has access to \\ less training data from certain \\ communities.\end{tabular}                                                     \\ \cline{2-4} 
\textbf{}                                                                   & \begin{tabular}[c]{@{}l@{}}Demographic \\ Blindness\end{tabular}                                     & \begin{tabular}[c]{@{}l@{}}The acts of treating \\ different individuals and \\ groups uniformly when \\ that  uniformity is not \\ warranted.\end{tabular}                                                                                                                                                                    & \begin{tabular}[c]{@{}l@{}}Ignoring   linguistic differences \\ when such differences exist may \\ further intensify disparities in \\ system outcomes for different   \\ language variants while making \\ it difficult to acknowledge the \\ resulting gaps.\end{tabular}                                                                    \\ \cline{2-4} 
\textbf{}                                                                   & \begin{tabular}[c]{@{}l@{}}Bias  \\ Amplification\end{tabular}                                       & \begin{tabular}[c]{@{}l@{}}The acts of amplifying \\ pre-existing inequities \\ and marginalization.\end{tabular}                                                                                                                                                                                                              & \begin{tabular}[c]{@{}l@{}}An expert identification system \\ may have certain demographic \\ biases, but these  biases may be \\ further amplified in terms of \\ exposure bias when the system’s   \\ predictions are presented as a \\ ranked list under heavy position \\ bias in how users inspect the \\ presented results.\end{tabular} \\ \hline
\end{tabular}
\end{table}
